Interactive Humanoid: Online Full-Body Motion Reaction Synthesis with Social Affordance Canonicalization and Forecasting

We focus on the human-humanoid interaction task optionally with an object. We propose a new task named online full-body motion reaction synthesis, which generates humanoid reactions based on the human actor's motions. The previous work only focuses on human interaction without objects and generates body reactions without hand. Besides, they also do not consider the task as an online setting, which means the inability to observe information beyond the current moment in practical situations. To support this task, we construct two datasets named HHI and CoChair and propose a unified method. Specifically, we propose to construct a social affordance representation. We first select a social affordance carrier and use SE(3)-Equivariant Neural Networks to learn the local frame for the carrier, then we canonicalize the social affordance. Besides, we propose a social affordance forecasting scheme to enable the reactor to predict based on the imagined future. Experiments demonstrate that our approach can effectively generate high-quality reactions on HHI and CoChair. Furthermore, we also validate our method on existing human interaction datasets Interhuman and Chi3D.

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{979} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2024}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{\small{Interactive Humanoid: Online Full-Body Motion Reaction Synthesis with Social Affordance Canonicalization and Forecasting}}  % **** Enter the paper title here
% \maketitle
% \vspace{-10mm}
% % \thispagestyle{empty}
% % \appendix
% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
% We thank all reviewers for all constructive comments. We will carefully proofread the paper and improve the presentation. 
% We are ready to release the dataset and code.

% % We express our gratitude to the reviewers for their constructive feedback. We commit to meticulously proofreading the paper to improve its presentation. Additionally, we are prepared to release both the dataset and the code.

% \noindent \textbf{Notation:} \textbf{\textcolor{magenta}{R1[99Fr] }\textcolor{blue} {R2[5RwD] }\textcolor{cyan} {R3[Bz7w] }\textcolor{red}{R4[ZAci]}}.

% \noindent\textbf{\textcolor{magenta}{R1}\textcolor{blue}{R2}\textcolor{cyan}{R3}\textcolor{red}{R4}: Regarding the presentation of Section 4.3.} We are refining the presentation for clearer alignment between figures and text. we will replace Figure 3 with this figure (please zoom in due to space limitations). The only difference between HHI and HHOI is the carrier selection process in Section 4.1, where carriers are represented by sparse point clouds (1024 points for objects, 475 points for human templates from SMPL-X) instead of key points. Additionally, a GNN maps human poses to embeddings, focusing on individual poses rather than entire motion sequences. During offline training, we fix the sequence length to 250 and add masks to future actor motions. For online prediction, the network only predicts one frame at each timestamp. 
% % We will carefully fix the presentation related issues.
% % To correspond the figure with the text more clearly, we will replace Figure 3 with this figure (please zoom in due to space limitations). The only difference between HHI and HHOI is the carrier selection process in Section 4.1, and the carrier is represented by a sparse point cloud (1024 points for objects and 475 points for human templates from SMPL-x) instead of key points. 
% % GNN is used to map a human pose to an embedding instead of the whole motion sequence.
% % For offline training, the sequence length $L$ is fixed to 250 and we add masks to future actor motions.  For online prediction, the network only predicts one frame at each timestamp. 





% % Human motion sequences are denoted as $s \in \mathbb{R}^{L \times J \times D}$, where $J$ is the number of joints(22 for the body and 32 for both hands) and $D_h$ refers to the position and velocity of each joint. 
% % For the carrier, we use the world frame. For the reactor, we use the point-wise local frame from the carrier.

%  % \vspace{-2mm}
% \begin{figure}[h]
%     \centering
%       \vspace{-3mm}
%     \includegraphics[width=1\linewidth]{4.3.jpg}
%     % \caption{Enter Caption}
%     \label{fig:4.3}
%     \vspace{-8mm}
% \end{figure}



% % We correspond the figure with the text in Sec. 4.3. But I cannot figure out what is the main difference with/without object from this figure.  whether the topology/skeleton of the object is assumed to be known or not? That is to say, at t=1, you have input {x1}, and at t=10, you have input {x1, x2, ..., x10}. These two sets does not have consistent dimensions as the input to GNN. 



% \noindent\textbf{\textcolor{magenta}{R1}\textcolor{blue}{R2}\textcolor{cyan}{R3}\textcolor{red}{R4}: Regarding the quality of our datasets.}  
% Our motion capture system has a high accuracy of 0.019 mm, effectively capturing contact regions as demonstrated in the figures below. We have thoroughly inspected the dataset to ensure its quality, and it is now ready for release.

% % Our mocap system has an accuracy of 0.019 mm and the contact region can be well depicted as shown by the figures below. The dataset has been manually inspected to guarantee the quality and is ready to be released.

% % We visualize the quality of the HHI and CoChair datasets, and it can be seen that our dataset has very high accuracy in contact. 

% % Although there is still room for improvement in the hand movements and contacts, our method has already made significant progress compared to existing methods.

% \begin{figure}[h]
%     \centering
%      \vspace{-3mm}
%     \includegraphics[width=1.0\linewidth]{vis.jpg}
%     % \caption{Enter Caption}
%         \vspace{-8mm}
%     \label{fig:vis}
% \end{figure}

% % Regarding the penetration between the object and humans.
% % The paper's claim of high-quality full-body motion synthesis is overshadowed by the unnatural hand motions observed in some of the video results on the provided website, particularly evident in the CoChair results that involve hand-object contacts. In some sequences, the hands keep an unnatural pose for most frames. When hand-object is involved, the hand does not grasp the object naturally and often show penetration. Moreover, it's not clear whether these artifacts already exist in the dataset or they are caused by the generation method. To clarify this, I recommend to also visualize the motion sequences in the collected datasets.





% % \noindent\textbf{\textcolor{magenta}{R1}: References of some terms.} Social affordance representation and affordance learning are broad concepts, commonly used in the field of human-object and human-human interaction, and we will add the references.

% \noindent\textbf{\textcolor{magenta}{R1}: 
% Only the history motion as input for social affordance forecasting.} We omit the reactor's influence on the actor's future motion, operating under the assumption that the actor's actions are primarily driven by a clear goal, a common scenario during the interaction. The reactor's role is considered secondary and is currently excluded. Modeling such a secondary factor is an interesting future work.

% % We consider the actors to have clear goals, without considering the impact of the reactors' motion on the actors. We think this higher-order social reaction is also valuable and interesting, which can be considered for future work.

% % We do not consider the reactor’s action influence on the actor’s future motion since we assume the actor has a clear goal dominating his action, which is the case in most assistive situations. The reactor’s action only plays a secondary role and is omitted for now. Modeling such a secondary factor is an interesting future work.

% \noindent\textbf{\textcolor{blue}{R2}: Regarding the local frame.} 
% The local frame, defining a new coordinate system, is determined by the point-wise orientation of its local region. Our SE(3)-equivariant network distinguishes between invariant scalar features, which remain constant, and equivariant vector features, which vary under SE(3) transformations. To ensure strict SE(3) equivariance, both $H_{in}$ and $V_{in}$ are set to zero. With Schmidt orthogonalization, the third direction can be derived, giving $v_{out,j}$.  For a local region, the equivariant network can output any orientation while ensuring equivariance. We expect the network to learn an orientation that is optimal for downstream tasks and can be generalized across objects.

% % Local frame refers to a point-wise orientation based on its local region which defines a new coordinate system. The SE(3)-equivariant network ensures the equivariance between the local frame and the object motion. Invariant scalar features refer to features that remain unchanged under different SE(3) transformations, while equivariant vector features change. These two features are very common in existing equivariant networks. $H_{in}$ and $V_{in}$ are all zeros to ensure the strict SE(3) equivariance of the network. When two directions are obtained, we can obtain the third direction through Schmidt orthogonalization, so $v_{out,j}$ has a 2x3 shape. For a local region, the equivariant network can output any orientation while ensuring equivariance. We expect the network to learn an orientation that is optimal for downstream tasks and can be generalized across objects.

% \noindent\textbf{\textcolor{blue}{R2}: Regarding transferring knowledge from HHI to HRI.}  We fully acknowledge the differences between humans and humanoid robots. As clarified in the footnote, our use of 'humanoid' specifically denotes virtual characters in AR/VR, not actual robots. We think studying human-human interactions is valuable for developing representation and network frameworks. Additionally, human-like demonstrations offer enhanced interpretability and facilitate smoother simulation-to-reality (sim2real) transfer.
% % We fully acknowledge the differences between humans and humanoid robots, so we mentioned in the footnote humanoid refers to virtual characters for AR/VR rather than real robots. We believe studying human-human interaction has reference significance in terms of representation and network framework, and human-like demonstration has advantages on interpretability and sim2real transferability.

% % \noindent\textbf{\textcolor{blue}{R2}:Reason for choosing the chair.} We think chairs have more diversity in geometry and are very common in our lives. At the same time, we plan to add more object categories in the future, such as tables and boxes.


% % \noindent\textbf{\textcolor{blue}{R2}\textcolor{red}{R4}:Regarding the humanoid reactor sequence $s_r$.} Humanoid reactor sequence are denoted as $s_r \in \mathbb{R}^{L \times J \times 6}$, where J is the number of joints(22 for body and 32 for both hands) and 6 refers to the joint position and velocity.



% \noindent\textbf{\textcolor{blue}{R2}: Details about motion classifier.}
% Following previous work, our approach utilizes a 4D motion encoder comprising a 4D convolution and a Transformer for feature extraction. We only train and test the classifier on the reaction part of the interaction, so the results are not influenced by the action. Classifying human interactions solely based on reactor motions introduces greater ambiguity and challenge, leading to relatively lower accuracy in classification. Additionally, the definition of motion classes is dataset-specific.
% %, which is always the ground truth.
% % Followed by other human motion generation works, we adopted a 4D motion encoder to extract features, which consists of a 4D convolution and a Transformer. We only train and test the classifier on the reaction part of the interaction, so the results are not influenced by the action, which is always the ground truth. Classifying human interactions only based on reactor motions becomes more ambiguous and challenging.  Consequently, the accuracy of such classification is relatively low. And the motion classes are determined by each dataset. 

% \noindent\textbf{\textcolor{blue}{R2}\textcolor{cyan}{R3}:Regarding the user preference score.} 
% For each test, 30 participants are presented with five videos with a label/description. Their task is to identify the most realistic one. Due to the lower quality of all current methods compared to real data, we decided not to include the real data.
% % The users are given five videos with the corresponding label/description. 30 participants need to choose the most realistic one. The quality of all current methods is significantly inferior to real data, so we have not considered the real dataset.





% \noindent\textbf{\textcolor{red}{R4}: Regarding the local frame for HHI.} 
% The presence of muscle leads to asymmetry in joint areas, which we'll highlight in the main paper. Visualizations of these learned local frames on various human templates are provided below.
% % Each human template is represented by a sparse point cloud instead of key points. The orientation of each point is determined by its local region, and due to the presence of muscles, most joint areas are not symmetrical, which we will emphasize in the main paper. We provide the visualization of learned local frames across different human templates below.

% \noindent\textbf{\textcolor{red}{R4}: Regarding the local frame for HHOI.} The local frame effectively captures both the object's local geometry and the actor's motion, creating a dense correlation between them which the global frame cannot achieve. Experiments starkly illustrate this: the local frame achieves a 0.9 cm penetration depth, surpassing the global frame's 2.8 cm and the point-wise global frame's 1.8 cm, which indicates the local frame's significant superiority. The learned local frames across different objects are shown below.
% % The local frame not only comprehends the local geometry of the object but also characterizes actor motion from various local perspectives. This densely establishes the correlation between object and actor motion, which is impossible using the global frame. Experimental results reveal a striking contrast: while the local frame achieves a 0.9 cm penetration depth, a global frame reaches 2.8 cm, and further, substituting it with a point-wise global frame leads to a 1.8 cm penetration depth, which indicates the learned local frame is significantly superior to the global frame.  The learned local frames across different objects are shown below.
% \begin{figure}[h]
%     \centering
%      \vspace{-3mm}
%     \includegraphics[width=1\linewidth]{frame.jpg}
%     % \caption{Enter Caption}
%     \vspace{-8mm}
%     \label{fig:frame}
% \end{figure}

% % Compared to the global frame, we believe the local frame can model the potential contact between the local regions and the actor. 
% % The local frame, derived from an object's local geometry, demonstrates enhanced generalization across different objects with similar geometries. 
% % The local frame is extracted based on local geometry, which has better generalization abilities between different objects with the same local geometry. 
% % We conduct experiments using only one global frame. Compared to the 0.9 cm penetration depth obtained by the local frame, a single global frame can only reach 2.8 cm. We further replace the point-wise local frame with the point-wise global frame, in which case only 1.8 cm penetration depth is achieved 
% \noindent\textbf{\textcolor{red}{R4}: Regarding generalization result on unseen objects.} 
% Each Object is represented by a point cloud instead of key points. In Table 3, we allocated five chairs to the training set and three to the test set, showcasing our network's performance on unseen objects. It indicates that our network successfully learns to correlate local geometry with an appropriate frame, achieving notable generalizability.
% % even with a limited training set.
% % For table 3, we divided 5 chairs into the training set and 3 chairs into the test set. The results have already demonstrated the performance of unseen objects. This indicates our network can learn how to relate local geometry with a proper frame, allowing it to acquire generalizability with just a small number of training objects.

% % Each object is represented by a sparse point cloud instead of key points. 
% % We believe the local frame is beneficial for generalization because it characterizes the potential contact between local geometry and actor motions.

% % We believe the local frame based on the sparse object point cloud is beneficial for generalization between different objects because it characterizes the potential contact between local geometry and actor motions. 
% % We also visualize the consistency of local frames across different objects in the figure (taking two points as examples).








% % \noindent\textbf{\textcolor{red}{R4}: Regarding the coordinate frames for carrier and reactor.}
% % For the carrier, we use the world frame. For the reactor, we use the point-wise local frame from the carrier.


% % \noindent\textbf{\textcolor{red}{R4}: Regarding the the online prediction process.}
% % During inference, the network only predicts one frame at each timestamp. The forecasting length($L$) used in experiments is 250 and the M just refers to the current timestamp.



























% % \noindent\textbf{\textcolor{magenta}{R1}\textcolor{red}{R4}: Social affordance forecasting in online setting.}

% % \noindent\textbf{\textcolor{blue}{R2}\textcolor{red}{R4}: Generation results on unseen objects.}

% % \noindent\textbf{\textcolor{blue}{R2}\textcolor{cyan}{R3}: User preference score.}

% % \noindent\textbf{\textcolor{magenta}{R1}\textcolor{blue}{R2}: Reference of some terms is missing.}

% % \noindent\textbf{\textcolor{blue}{R2}\textcolor{red}{R4}: How many joints and what joint features are used to represent the body motion?}


% % \noindent\textbf{\textcolor{magenta}{R1}: Improve data quality considering the penetration.}

% % \noindent\textbf{\textcolor{blue}{R2}: Questions on SE(3)-Equivariance Netork.}

% % % \noindent\textbf{\textcolor{blue}{R2}: The term of HOI}:

% % \noindent\textbf{\textcolor{blue}{R2}: Transfer the knowledge learned from HHI to HRI.}

% % \noindent\textbf{\textcolor{blue}{R2}: The figures are too small}:

% % \noindent\textbf{\textcolor{blue}{R2}: Plan to extend the object categories}:

% % \noindent\textbf{\textcolor{blue}{R2}: What is sr exactly?}:



% % \noindent\textbf{\textcolor{blue}{R2}: Details of motion classifier.}

% % % \noindent\textbf{\textcolor{cyan}{R3}: Eq. 5: what is p?}:



% % \noindent\textbf{\textcolor{red}{R4}: The advantage of predicting local frame.}



% % \noindent\textbf{\textcolor{red}{R4}: Selection of the coordinate frames.}

% % \noindent\textbf{\textcolor{red}{R4}: The online prediction process}: 


% % %%%%%%%%% REFERENCES
% % {
% %     \small
% %     \bibliographystyle{ieeenat_fullname}
% %     \bibliography{main}
% % }

% \end{document}


==> sec/tupleinfonce_template.tex <==
\setcounter{section}{0}
\def\thesection{\Alph{section}}

This document provides a list of supplemental materials to support the main paper.
\begin{itemize}
    \item \textbf{Additional experiments and ablation studies}
    \begin{itemize}
    \item We provide additional experiments to explore whether the representation quality improves as the number of modalities increases in Section~\ref{sec:revisit}.
    \item We compare with a data augmentation search method InfoMin~\cite{tian2020makes} in Section~\ref{sec:augmentation_search}.
    \item We conduct experiments on the NYUv2 dataset with four input modalities in Section~\ref{sec:four}, to demonstrate the flexibility and efficacy of our framework in handling different numbers of input modalities.
    \item In Section~\ref{sec:ablation}, we validate the sampling efficiency of TupleInfoNCE by comparing with another negative sampling strategy.
    \end{itemize}
    \item \textbf{Proof for the MI lower bound of TupleInfoNCE} - In Section~\ref{sec:proof}, we provide a mathematical proof for the mutual information lower bound we maximize via optimizing the TupleInfoNCE objective.
    \item \textbf{More examples for sample optimizations}
    \begin{itemize}
        \item In order to further understand the negative sample optimization scheme, we provide the sampling ratio on each data set and provide an intuitive understanding of the results in Section~\ref{sec:sampling}.
        \item We provide the optimized data augmentation strategy on each data set to understand the efficacy of positive sample optimization in Section~\ref{sec:augmentation}.
    \end{itemize}
    \item\textbf{Additional technical details}
    \begin{itemize}
        \item In Section~\ref{sec:dropout}, we explain our dropout training strategy, which enables us to handle missing input modalities.
        \item We provide implementation details of our whole framework in Section~\ref{sec:implementation_details}.
    \end{itemize}
\end{itemize}

\section{Does representation quality improve as number of views increases?}
\label{sec:revisit}
To measure the quality of the learned representation, we consider the task of semantic segmentation on NYUv2. In the 1 modality setting case, TupleInfoNCE using RGB modality coincides with InfoNCE. In 2-3 modalities cases, we sequentially add depth and normal modalities.

\begin{table}[h]
\centering
\label{tab:revisit}
\begin{tabular}{c|c} 
    \toprule
    Modality & mIoU\\
    \midrule 
    RGB & 40.8  \\
    RGB + depth & 44.1  \\
    RGB + normal  & 44.5 \\
    depth + normal  & 46.3  \\
    RGB + depth + normal & \textbf{48.1}\\
    \bottomrule
\end{tabular}
\vspace{5pt}
\caption{We show the mean Intersection over Union (mIoU) for the NYU-Depth-V2 dataset, as TupleInfoNCE is trained with increasingly more modalities from 1 to 3. The performance steadily improves as new modalities are added.}
\end{table}

As shown in Tab.~\ref{tab:revisit}, We see that the performance steadily improves as new modalities are added. This finding is consistent with that of CMC~\cite{tian2019contrastive} who learn a cross-modal embedding space. 

\section{Comparisons to InfoMin}
\label{sec:augmentation_search}
% \noindent\textbf{Comparisons to Infomin}
Infomin~\cite{tian2020makes} proposes to reduce the mutual information between different views while retaining the task-relevant information as much as possible. But how to explore task-relevant information without labels is a very challenging problem. Infomin utilizes an adversarial training strategy to search for good views in a weakly-supervised manner. When no labels are available, which is the case in a truly self-supervised representation learning setting, the effectiveness of Infomin is greatly reduced.
% However, the generator has difficulty finding the direction of the task-relevant without any labels, so its effectiveness is greatly reduced. Additionally, guiding an unsupervised training process through supervised evaluations is not possible for real-world data that does not actually contain labels.
% We propose to use crossmodal discrimination as an evaluation approach which is completely in a self-supervised manner without any labels.
Taking NYUv2 semantic segmentation task as an example, in a truly self-supervised representation learning setting, the optimal rotation parameter Infomin finds is 70 degrees, which leads to 46.91 mIoU after downstream fine-turning, while the optimal rotation parameter TupleInfoNCE finds is 40 degree, corresponding to 47.41 mIoU. 
% Our method is specifically designed for multimodal tasks and cannot be applied directly to a single modality task. How to design an automatic mechanism to search a good view in singlemodal contrastive learning completely in self-supervised manner remain an open problem.

% \paragraph{Comparisons to SelfAugment}
% SelfAugment~\cite{metzger2020evaluating} points out evaluating the learned representations with a self-supervised image rotation task is highly correlated with a standard set of supervised evaluations. 

\section{Use TupleInfoNCE in four modalities}
\label{sec:four}
We conduct another experiment on NYUv2 to see whether our method can help multi-modal semantic scene understanding in the case of 4 modalities. Following CMC, modalities we used are L, ab, depth, normal. We follow the 3 modalities setting and use random cropping, rotation, and jittering as the augmentation strategy, thus learning a fused representation by contrasting tuples that contain 4 modalities. Using 4 modalities, the best mIoU we obtain is 48.6. This is 0.5 higher than our 3 modalities baseline, showing that our method has strong generalization ability. These again validate that our TupleInfoNCE which contrasts multi-modal input tuples can produce better-fused representations.

\section{Sampling efficiency of TupleInfoNCE}
\label{sec:ablation}
% \paragraph{Sample efficiency of TupleInfoNCE}
% Show how final accuracy changes w.r.t the negative sample size (batch size) using both TupleInfoNCE and naive tuple disturbing strategy.
% \eric{Need to explain what is the naive sampling baseline}
TupleInfoNCE disturbs each modality separately to generate k disturbed negative samples. However, The most direct method is the naive sampling strategy which disturbs all modalities simultaneously to generate 1 disturbed negative sample. We conduct another experiments to compare our method with the naive sampling strategy from the perspective of efficiency. Figure~\ref{fig:batchsize} shows that our method is more efficient than naive tuple disturbing strategy. Our method with a batch size of 512 already outperforms naive tuple disturbing strategy with a batch size of 1024.
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/batchsize.pdf}
    \caption{Sample efficiency of TupleInfoNCE}
    % \eric{update the legend to make TupleInfoNCE on the top}
    \label{fig:batchsize}
\end{figure}

\section{Proof for the MI lower bound of TupleInfoNCE}
\label{sec:proof}
The TupleInfoNCE loss is essentially a categorical cross-entropy classifying positive tuples $\bt_{2,i}\sim p_{\bbeta}(\bt_2|\bt_{1,i})$ from $N-1$ negatives views $\bt_{2,j}\sim q_{\balpha}(\bt_2)$. We use $p_{\balpha\bbeta}(d=i|\bt_{1,i})$ to denote the optimal probability for this loss where $[d=i]$ is an indicator showing that $\bt_{2,i}$ is the positive view. Then we can derive $p_{\balpha\bbeta}(d=i|\bt_{1,i})$ as follows:

\begin{equation*}
\begin{split}
    p_{\balpha\bbeta}(d=i|\bt_{1,i}) &= \frac{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})\prod_{l\neq i}q_{\balpha}(\bt_{2,l})}{\sum_{j=1}^Np_{\bbeta}(\bt_{2,j}|\bt_{1,i})\prod_{l\neq j}q_{\balpha}(\bt_{2,l})}\\
    &=\frac{\frac{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}{q_{\balpha}(\bt_{2,i})}}{\sum_{j=1}^N\frac{p_{\bbeta}(\bt_{2,j}|\bt_{1,i})}{q_{\balpha}(\bt_{2,j})}}
\end{split}
\end{equation*}

\noindent It can be seen from above that the optimal value for $f(\bt_{2,j},\bt_{1,i})$ in $\mathcal{L_{\text{TNCE}}(\balpha,\bbeta)}$ is proportional to $\frac{p_{\bbeta}(\bt_{2,j}|\bt_{1,i})}{q_{\balpha}(\bt_{2,j})}$. Insert this density ratio back to $\mathcal{L_{\text{TNCE}}(\balpha,\bbeta)}$ we get:

\begin{equation*}
\begin{split}
& \mathcal{L}_{\text{TNCE}}^{\text{OPT}}(\balpha,\bbeta)\\
=& -\mathbb{E}\,\text{log}\left[\frac{\frac{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}{q_{\balpha}(\bt_{2,i})}}{\frac{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}{q_{\balpha}(\bt_{2,i})}+\sum_{j\neq i}\frac{p_{\bbeta}(\bt_{2,j}|\bt_{1,i})}{q_{\balpha}(\bt_{2,j})}}\right]\\
=&\, \mathbb{E}\,\text{log}\left[1+ \frac{q_{\balpha}(\bt_{2,i})}{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}\sum_{j\neq i}\frac{p_{\bbeta}(\bt_{2,j}|\bt_{1,i})}{q_{\balpha}(\bt_{2,j})}\right]\\
\approx&\, \mathbb{E}\,\text{log}\left[1+ \frac{q_{\balpha}(\bt_{2,i})}{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}(N-1)\underset{\bt_{2,j}}{\mathbb{E}}\frac{p_{\bbeta}(\bt_{2,j}|\bt_{1,i})}{q_{\balpha}(\bt_{2,j})}\right]\\
=&\, \mathbb{E}\,\text{log}\left[1+ \frac{q_{\balpha}(\bt_{2,i})}{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}(N-1)\right]\\
\geq& \, \mathbb{E}\,\text{log}\left[\frac{q_{\balpha}(\bt_{2,i})}{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}N\right]\\
\end{split}
\end{equation*}

\noindent We design our negative ``proposal'' distribution as $q_{\balpha}(\bt_2)=\alpha_0p(\bt_2)+\sum_{k=1}^K\alpha_kp(\bar{\bv}_2^k)p(\bv_2^k)$. Insert this to the inequality above we obtain:

\begin{equation*}
\begin{split}
& \mathcal{L}_{\text{TNCE}}^{\text{OPT}}(\balpha,\bbeta)\\
\geq& \, \mathbb{E}\,\text{log}\left[\frac{\alpha_0p(\bt_{2,i})+\sum_{k=1}^K\alpha_kp(\bar{\bv}_{2,i}^k)p(\bv_{2,i}^k)}{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}N\right]\\
\geq& \, \mathbb{E}\,\text{log}\left[\frac{(p(\bt_{2,i}))^{\alpha_0}\prod_{k=1}^K(p(\bar{\bv}_{2,i}^k)p(\bv_{2,i}^k))^{\alpha_k}}{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}N\right]\\
=& \, \mathbb{E}\,\text{log}\left[\frac{p(\bt_{2,i})}{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}\prod_{k=1}^K(\frac{p(\bar{\bv}_{2,i}^k)p(\bv_{2,i}^k)}{p(\bt_{2,i})})^{\alpha_k}N\right]\\
\approx & \, \mathbb{E}\,\text{log}\left[\frac{p_{\bbeta}(\bt_{2,i})}{p_{\bbeta}(\bt_{2,i}|\bt_{1,i})}\prod_{k=1}^K(\frac{p(\bar{\bv}_{2,i}^k)p(\bv_{2,i}^k)}{p(\bt_{2,i})})^{\alpha_k}N\right]\\
=& \, \text{log}(N)-I(\bt_{2,i};\bt_{1,i}|\bbeta)-\sum_{k=1}^K\alpha_kI(\bv_{2,i}^k;\bar{\bv}_{2,i}^k)
\end{split}
\end{equation*}

\noindent Therefore $I(\bt_{2,i};\bt_{1,i}|\bbeta)+\sum_{k=1}^K\alpha_kI(\bv_{2,i}^k;\bar{\bv}_{2,i}^k)\geq \text{log}(N)-\mathcal{L}_{\text{TNCE}}^{\text{OPT}}(\balpha,\bbeta)$.

\section{Examples for negative sample optimization}
\label{sec:sampling}
This paper sets out with the aim of assessing the importance of complementary synergies between modalities. What is surprising is that increasing the ratio of weak modalities which is considered to contain less useful information can produce better-fused multi-modal representations. To be specific, the negative sample sampling ratio is roughly 1(RGB): 2(depth): 3(normal) in NYUv2 semantic segmentation task, 1(text): 1(video): 4(audio) in MOSI/MOSEI sentiment analysis task, and 1(point cloud): 3(RGB color): 2(height) in SUNRGB-D 3D Object Detection task. These results further support our idea of contrasting multi-modal input tuples to avoid weak modalities being ignored and to facilitate modality fusion. A possible explanation for this might be that our proposed TupleInfoNCE encourages neural networks to use complement information in weak modalities, which can avoid networks converging to a lazy suboptimum where the network relies only on the strongest modality. This observation may support the hypothesis that mining useful information contained in weak modalities instead of always emphasizing strong modal information can obtain better fusion representations.

\section{Examples for positive sample optimization}
\label{sec:augmentation}
As mentioned in the main paper, we need to optimize the positive samples so that the contrastive learning can keep the shared information between positive and anchor samples while abstracting away nuisance factors. In the NYUv2 semantic segmentation task, rotation of 40 degrees, cropping with 160 center pixels, and Gaussian noise with a variance of 50 is best for RGB modality, while no augmentation is better for depth and normal modalities. As for the SUNRGB-D 3D Object Detection task, the final augmentation is to rotate the point cloud by 10 degrees, add Gaussian noise with a variance of 30 to the RGB image, and apply Gaussian noise with a variance of 10 to the height modality.

\section{Dropout training}
\label{sec:dropout}
\vspace*{2mm}\noindent\textbf{Dropout training}
Note $\bg^{\balpha\bbeta}$ is originally designed to consume all input modalities, while in the crossmodal discrimination task, $\bg^{\balpha\bbeta}$ needs to handle missing modalities as shown in Equation. We adopt a simple \textit{dropout training} strategy to achieve this goal. To be specific, we randomly mask out modalities and fill them with placeholder values in the input. The missing modalities are the same in the positive and negative samples, yet could be different in the anchor tuple. This dropout strategy is only adopted with a probability of 0.6 for each training batch and the rest of the time we feed complete inputs to the feature encoder.

\paragraph{Robustness to dropout training}
We found dropout training does not cause a drop in feature quality compared to non-dropout training. 
We first obtain the optimal hyper-parameter by grid searching. When we use a dropout training strategy with fixed optimal hyper-parameter in NYUv2 semantic segmentation task, we achieve 48.3 mIoU performance which only outperforms our strategy by $0.2\%$, which presumably means dropout training might distill information from other modalities to avoid representation quality degradation. 
% \eric{Need to show dropout training does not influence the learned representations through optimizing TupleInfoNCE, rather than the train from scratch baseline.}

\section{Implementation Details}
\label{sec:implementation_details}
For NYU-Depth-V2 semantic segmentation task, we train the model with one V100 GPU for 500 epochs. The batch size is 20. We use SGD+momentum optimizer with an initial learning rate 0.25. We use onecycle learning rate scheduler. We set the weight decay as 1e-4. In the experiment of SUN RGB-D 3D object detection, our settings are consistent with VoteNet. We train the model on one 2080Ti GPU for 180 epochs. The initial learning rate is 0.001. We sample 20,000 points from each scene and the voxel size is 5cm. As for sentiment analysis on MOSEI and MOSI,  We used the same data as MISA, where text features are extracted from BERT. Batch size is 32 for MOSI, and 16 for MOSEI.
For sample optimization details, we provide a flow chart Figure~\ref{fig:optimaize} to further support the main paper.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{./figures/optimize.pdf}
    \caption{Overview of sample optimization.}
    \label{fig:optimaize}
    \vspace{-15pt}
\end{figure}






